OPlaceRAN -- a Placement Orchestrator for Virtualized Next-Generation of Radio Access Network

The fifth-generation mobile evolution enables transformations on Next-Generation Radio Access Networks (NG-RAN). The RAN protocol stack is split into eight disaggregated options combined in three network units, i.e., Central, Distributed, and Radio. Besides that, further advances allow the RAN functions to be virtualized on top of general-purpose hardware, using the concept of virtualized RAN (vRAN). The Combination of NG-RAN and vRAN results in vNG-RAN, which enables the management of the disaggregated units and protocols as a set of radio functions. However, the orchestration-based placement of these radio functions is a challenging issue since the best decision can be determined by multiple constraints involving RAN disaggregation, crosshaul networks requirements, availability of computational resources, etc. This article proposes OPlaceRAN, a vNG-RAN deployment orchestrator framed within the NFV reference architecture and aligned with the Open RAN initiative. OPlaceRAN supports the dynamic placement of radio functions focusing on vNG-RAN planning and is designed to be agnostic to the placement optimization model. To validate OPlaceRAN, we developed a prototype based on up-to-date cloud-native tools to deploy RAN using containerized virtualization using the OpenAirInterface emulator and considering two distinct functional splits (options 2 and 6). The evaluation is tested as proofs-of-concept in a real computing infrastructure using two different placement solutions. Our results reveal that OPlaceRAN is an effective cloud-native solution for containerized network functions placement and agnostic to the optimization model. Additionally, OPlaceRAN is up-to-date with the most advanced vNG-RAN design and development approaches, contributing to the evolution of the fifth-generation of mobile networks.

==> Tables/functional_split.tex <==

%% Comentário do Contreras 
% Probably good to add reference of the scpecification from 3GPP from where this table is taken.
\begin{table}[!h]
   \caption{3GPP Latency and bitrate requirements for each split based on correspond to an RU with the following configuration: 100 MHz bandwidth of spectrum, 32 antenna ports, 8 MIMO layers, and 256 QAM modulation \cite{3gpp2017study}.}
    \label{tab:splits}
    \centering{ {
        \begin{tabular}{|c|l|c|c|c|}
        \hline
    Split & \multicolumn{1}{c|}{Functional} & One-way & \multicolumn{2}{c|}{Bitrate (Gbps)} \\ 
    \cline{4-5}
    Option & \multicolumn{1}{c|}{Split} & latency & DL & UL \\ \hline
    
    \rowcolor[HTML]{cdd5e4}  O1 &  RRC-PDCP      & 10 ms      & 4    & 3  \\
    
    O2 & PDCP - High RLC  & 10 ms      & 4    & 3  \\
    
    \rowcolor[HTML]{cdd5e4} O3 & High RLC -  Low RLC & 10 ms      & 4    & 3  \\ 
    
    O4 & Low RLC - High MAC  & 1 ms      & 4  & 3  \\ 
    
    \rowcolor[HTML]{cdd5e4} O5 & High MAC - Low MAC & $<$ 1 ms   & 4  & 3  \\ 
    
    O6 & Low MAC - High PHY & 250 $\mu$s & 4.13  & 5.64  \\ 
    
    \rowcolor[HTML]{cdd5e4} O7 & High PHY - Low PHY & 250 $\mu$s & 86.1$^*$  & 86.1$^*$  \\ 
    
    O8 & Low PHY - RF & 250 $\mu$s & 157.3 & 157.3 \\ \hline
    
       \end{tabular}
       O7 split maximum value.$^*$ 
    } }
\end{table}

% \begin{table}[!h]
%   \caption{Latency and bitrate requirements for each split.}
%   % \textcolor{red}{discutir deixar os valores do 3GPP, para não gerar conflitos com a tabela da avaliação.}
%     \label{tab:splits}
%     \centering{ {
%         \begin{tabular}{|c|l|c|c|c|}
%         \hline
%     Split & \multicolumn{1}{c|}{Functional} & One-way & \multicolumn{2}{c|}{Bitrate (Gbps)} \\ 
%     \cline{4-5}
%     Option & \multicolumn{1}{c|}{Split} & latency & DL & UL \\ \hline
    
%     \rowcolor[HTML]{cdd5e4}  O1 &  RRC-PDCP      & 10 ms      & 4    & 3  \\
    
%     O2 & PDCP - High RLC  & 10 ms      & 4    & 3  \\
    
%     \rowcolor[HTML]{cdd5e4} O3 & High RLC -  Low RLC & 10 ms      & 4    & 3  \\ 
    
%     O4 & Low RLC - High MAC  & 1 ms      & 5.2  & 4.5  \\ 
    
%     \rowcolor[HTML]{cdd5e4} O5 & High MAC - Low MAC & $<$ 1 ms   & 5.6  & 7.1  \\ 
%     O6 & Low MAC - High PHY & 250 $\mu$s & 5.6  & 7.1  \\ 
    
%     \rowcolor[HTML]{cdd5e4} O7 & High PHY - Low PHY & 250 $\mu$s & 9.8  & 15.2  \\ 
    
%     O8 & Low PHY - RF & 250 $\mu$s & 157.3 & 157.3 \\ \hline
    
%       \end{tabular}
%     } }
% \end{table}
